LATIS: Lambda Abstraction-based Thermal Image Super-resolution

Single image super-resolution (SISR) is an effective technique to improve the quality of low-resolution thermal images. Recently, transformer-based methods have achieved significant performance in SISR. However, in the SR task, only a small number of pixels are involved in the transformers self-attention (SA) mechanism due to the computational complexity of the attention mechanism. The lambda abstraction is a promising alternative to SA in modeling long-range interactions while being computationally more efficient. This paper presents lambda abstraction-based thermal image super-resolution (LATIS), a novel lightweight architecture for SISR of thermal images. LATIS sequentially captures local and global information using the local and global feature block (LGFB). In LGFB, we introduce a global feature extraction (GFE) module based on the lambda abstraction mechanism, channel-shuffle and convolution (CSConv) layer to encode local context. Besides, to improve the performance further, we propose a differentiable patch-wise histogram-based loss function. Experimental results demonstrate that our LATIS, with the least model parameters and complexity, achieves better or comparable performance with state-of-the-art methods across multiple datasets.

==> sec/ab_table1.tex <==
\begin{table}[htb]
\caption{Effectiveness of the lambda layer in GFE module.}
\label{tab:vit}
%\hspace*{1em}
\begin{tabularx}{0.48\textwidth} 
{ 
   >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  >{\centering\arraybackslash}X  }
 \hline
 Structure & w/ Self-Attention & w/ Lambda Layer\\
 \hline
 PSNR/SSIM & 35.84/0.9345 & \textbf{37.91}/\textbf{0.9596}\\
 \hline
 Params (K) & 98 & 193\\
 \hline
 FLOPs (G) (K) & 0.35 & 0.37\\
 \hline
\end{tabularx}
\end{table}

==> sec/lambda_algo.tex <==
\begin{algorithm*}
\caption{Pseudo code for the lambda layer}
\label{alg:lambda}
\KwIn{$\text{query} \in\mathbb{R}^{\text{b,\:k,\:h,\:hh,\:ww}}$}
\KwIn{$\text{key} \in\mathbb{R}^{\text{b,\:k,\:u,\:hh,\:ww}}$}
\KwIn{$\text{value} \in\mathbb{R}^{\text{b,\:v,\:u,\:hh,\:ww}}$}
\KwOut{$\text{output} \in\mathbb{R}^{\text{b,c,hh,ww}}$}
\#\: k: query/ key depth \\
\#\: v: value depth \\
\#\: h: number of heads \\
$\text{content}\_\text{lambda} \gets$ einsum\:(softmax\:(key), value,\:'b\:u\:k\:m,\:b\:u\:v\:m\:$->$ \:b\:k\:v')\\
$\text{position}\_\text{lambda} \gets$ positional\_encoding\:(value) \\
$\text{content}\_\text{output}\gets$ einsum\:(query, $\text{content}\_\text{lambda}$,\:'b\:h\:k\:n,\:b\:k\:v\:$->$ \:b\:h\:v\:n')\\
$\text{position}\_\text{output}\gets$ einsum\:(query, $\text{position}\_\text{lambda} $,\:'b\:h\:k\:n,\:b\:k\:v\:n\:$->$ \:b\:h\:v\:n')\\
$\text{output} \gets \text{content}\_\text{output}\:+\:\text{position}\_\text{output}$\\
$\text{output} \gets$ rearrange\:($\text{output}$,\:'b\:h\:v\:(hh\:ww)\:$->$\:b\:(h\:v)\:hh\:ww\:')
\end{algorithm*}



\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/rgb_image_2000.png}
        \caption{RGB image}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/lr_image_2000.png}
        \caption{Thermal LR}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/bicubic_2000.png}
        \caption{Bicubic}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/LBNet_2000.png}
        \caption{LBNet \cite{lbnet}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/shuffleMixer_2000.png}
        \caption{ShuffleMixer \cite{shuffleMixer}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/UGSR_FA_2000.png}
        \caption{UGSR-FA \cite{ugsr}}
        \label{fig:gull}
    \end{subfigure}
    %\vfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/UGSR_ME_2000.png}
        \caption{UGSR-ME \cite{ugsr}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/DCTNet_2000.png}
        \caption{DCTNet \cite{dctnet}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/MMSR_2000.png}
        \caption{MMSR \cite{mmsr}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/DAT_2000.png}
        \caption{DAT \cite{dat}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/ours_2000.png}
        \caption{Ours}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.16\textwidth}
       \includegraphics[width=\textwidth]{sec/images/x4/ground_truth_2000.png}
        \caption{Thermal HR}
        \label{fig:gull}
    \end{subfigure}
    \caption{Visual comparison for x4 SR on KAIST datasets. The proposed algorithm recovers the image with a clearer structure.}
    \label{fig:fig6}
\end{figure*}

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{sec/images/loss_x4/ground_truth_3500.png}
        \caption{Ground Truth}
        \label{fig:gull}
    \end{subfigure}
    \hfill    
    \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{sec/images/loss_x4/ours_only_L1_3500.png}
        \caption{Training with 
$\mathcal{L}_C$\:loss}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
       \includegraphics[width=\textwidth]{sec/images/loss_x4/ours_L1_and_EMD_3500.png}
        \caption{Training with 
$\mathcal{L}_C+\lambda\mathcal{L}_P$\:loss}
        \label{fig:gull}
    \end{subfigure}
    \caption{Visual comparison for EMD loss for x4 SR on FLIR-ADAS test set. Training with $\mathcal{L}_C+\lambda\mathcal{L}_P$\:loss recovers the image with a clearer structure.}
    \label{fig:loss_compare}
\end{figure}

\begin{table}[hbt!]
\caption{Results for the channel shuffling, layer norm, and CBAM modules on the x2 CATS test set. The best results are highlighted.}
\centering
\begin{tabular}{CCCCC}
\toprule
\multicolumn{1}{c}{\makecell{Channel \\ Shuffling}} & \multicolumn{1}{c}{\makecell{Layer \\ Norm}} & \multicolumn{1}{c}{CBAM} & \multicolumn{1}{c}{PSNR (dB)} & \multicolumn{1}{c}{SSIM} \\
\midrule
\multirow{1}{*}{\xmark} & \multirow{1}{*}{\cmark} & \multirow{1}{*}{\cmark}& \multirow{1}{*}{37.75}& \multirow{1}{*}{0.9580}\\
\multirow{1}{*}{\cmark} & \multirow{1}{*}{\xmark} & \multirow{1}{*}{\cmark}& \multirow{1}{*}{35.83}& \multirow{1}{*}{0.9384}\\
\multirow{1}{*}{\cmark} & \multirow{1}{*}{\cmark} & \multirow{1}{*}{\xmark}& \multirow{1}{*}{37.77}& \multirow{1}{*}{0.9589}\\
\multirow{1}{*}{\cmark} & \multirow{1}{*}{\cmark} & \multirow{1}{*}{\cmark}& \multirow{1}{*}{\textbf{37.91}}& \multirow{1}{*}{\textbf{0.9596}}\\
\bottomrule
\end{tabular}
\label{tab:comp}
\end{table}



==> sec/visual3.tex <==
\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{RGB image/ Thermal LR}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{Bicubic}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{LBNet \cite{lbnet}}
        \label{fig:gull}
    \end{subfigure}
    \caption{Visual comparison on an image from CATS test set for x3 SR.}
    \label{fig:v3}
\end{figure*}

==> sec/visual4.tex <==
\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{RGB image/ Thermal LR}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{Bicubic}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{LBNet \cite{lbnet}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{ShuffleMixer \cite{shuffleMixer}}
        \label{fig:gull}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{DAT \cite{dat}}
        \label{fig:gull}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
       \includegraphics[width=\textwidth]{sec/images/hist1/ground_truth_hist.png}
        \caption{Ours}
        \label{fig:gull}
    \end{subfigure}
    \caption{Visual comparison on an image from CATS test set for x3 SR.}
    \label{fig:v3}
\end{figure*}
